Statistical Mechanics of Household Income and Wealth: Derivation from Firm Dynamics via Maximum Entropy and Mixture Aggregation

The distribution of income and wealth in developed economies exhibits a robust two-class structure: an exponential (Boltzmann--Gibbs) bulk covering $\sim\!97\%$ of the population, and a power-law (Pareto) tail in the upper $\sim\!3\%$. We derive this structure from first principles via an explicit mechanistic chain: Gibrat's law for firm growth implies a Zipf firm-size distribution; maximum entropy applied to within-firm wages, combined with mixture aggregation across firms, yields a Boltzmann--Gibbs income distribution with temperature $T_y$ for employees; additive-noise wealth dynamics with a reflecting wall at zero produce a Boltzmann--Gibbs employee wealth distribution with temperature $T_w$. For firm owners, multiplicative capital returns produce a Pareto wealth tail with exponent $\alpha_w = 1/\theta$, where $\theta$ encodes how total returns scale with firm size. The empirical value $\alpha_w \approx 1.30$ \cite{Yakovenko2009} is reproduced with no tuned parameters from the observed firm value scaling $V = V_0(s/s_0)^{0.77}$~\cite{Axtell2001}, and simultaneously yields the first quantitative estimate of the returns-per-employee size exponent: $\zeta = \theta - 1 \approx -0.23$. For empirical values $\nu \approx 0.3$, $c \approx 0.81$, $k \approx 0.15$ (BEA long-run savings rate $\approx 5\%$), the model gives $T_w/T_y \approx 1.7\,\text{yr}$, i.e.\ lower-class households hold roughly 1--2 years of income as wealth, with the precise ratio depending on savings and tax rates and testable cross-country. As a parameter-free empirical test, firms near zero profit have a cash martingale whose first-passage time gives establishment exit rate $\sim t^{-1/2}$; convolving with the Zipf firm-size distribution yields firm-level exit rate $\sim t^{-1/2}\!\log t$, with apparent exponent $b = 0.295 \pm 0.03$, confirmed against BDS firm-age data with no free parameters.

==> Fig1_01.tex <==
\begin{tikzpicture}[x=1cm, y=1cm]

% ════════════════════════════════════════════════════════════
%  LEFT PANEL (a)
% ════════════════════════════════════════════════════════════

% (bounding box removed)

%% ── Sector boxes ──────────────────────────────────────────

% Firms
\draw[draw=bordergray, fill=boxgray, rounded corners=4pt, line width=0.4pt]
  (0.30, -0.42) rectangle (5.70, 0.42);
\node[font=\small, align=center] at (3.00, 0.14)
  {\textbf{Firms}};
\node[font=\scriptsize] at (3.00, -0.17)
  {Zipf size distribution};

% Households (outer) — white fill
\draw[draw=bordergray, fill=white, rounded corners=5pt, line width=0.4pt]
  (0.30, -4.485) rectangle (5.70, -1.985);
\node[font=\small] at (3.00, -2.255)
  {\textbf{Households}};

% Employees sub-box
\draw[draw=bordergray, fill=boxgray, rounded corners=3pt, line width=0.4pt]
  (0.45, -4.285) rectangle (2.75, -2.685);
\node[font=\footnotesize] at (1.60, -2.935)
  {\textbf{Employees}};
\node[font=\tiny] at (1.60, -3.285)
  {$\oplus$ additive wages};
\node[font=\tiny] at (1.60, -3.585)
  {BG income};
\node[font=\tiny] at (1.60, -3.905)
  {BG wealth};

% Owners sub-box
\draw[draw=bordergray, fill=boxgray, rounded corners=3pt, line width=0.4pt]
  (3.25, -4.285) rectangle (5.55, -2.685);
\node[font=\footnotesize] at (4.40, -2.935)
  {\textbf{Owners}};
\node[font=\tiny] at (4.40, -3.285)
  {$\otimes$ multiplicative};
\node[font=\tiny] at (4.40, -3.585)
  {Pareto income};
\node[font=\tiny] at (4.40, -3.905)
  {Pareto wealth};

% Government
\draw[draw=bordergray, fill=boxgray, rounded corners=4pt, line width=0.4pt]
  (0.30, -6.90) rectangle (5.70, -6.05);
\node[font=\small] at (3.00, -6.34)
  {\textbf{Government}};
\node[font=\scriptsize] at (3.00, -6.67)
  {fiscal flows (invariant)};

%% ── SOLID arrows ──────────────────────────────────────────

% Wages
\draw[solidarr] (1.60, -0.42) -- (1.60, -2.685);
\node[elabel] at (1.60, -1.202) {wages};

% Consumption
\draw[solidarr] (3.00, -1.985) -- (3.00, -0.42);
\node[elabel] at (3.00, -1.202) {consumption};

% Returns
\draw[solidarr] (4.40, -0.42) -- (4.40, -2.685);
\node[elabel] at (4.40, -1.202) {returns};

%% ── DASHED arrows ─────────────────────────────────────────

% HH taxes
\draw[dasharr] (3.00, -4.485) -- (3.00, -6.05);
\node[elabel] at (3.00, -5.268) {hh taxes};

% Firm taxes: right margin
\draw[dasharr]
  (5.70,  0.00) -- (6.25,  0.00)
               -- (6.25, -6.48)
               -- (5.70, -6.48);
\node[elabel, rotate=90] at (6.25, -3.24) {firm taxes};

% Spending: left margin
\draw[dasharr]
  (0.30, -6.48) -- (-0.25, -6.48)
               -- (-0.25,  0.00)
               -- ( 0.30,  0.00);
\node[elabel, rotate=90] at (-0.25, -3.24) {spending};

%% ── Panel label ───────────────────────────────────────────
\node[font=\small] at (3.00, -7.55) {(a)};


% ════════════════════════════════════════════════════════════
%  RIGHT PANEL (b)
% ════════════════════════════════════════════════════════════

\def\XO{6.85}   % panel x start
\def\xL{7.45}   % plot left edge
\def\xR{12.85}  % plot right edge
\def\W{5.40}    % plot width
\def\H{1.80}    % plot height
\def\pitch{2.65}% vertical pitch
\def\f{0.50}    % x* fraction

% (bounding box removed)

\pgfmathsetmacro{\xst}{\xL+\f*\W}

%% ┄┄ PLOT 1: firm size ┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄

\def\yT{0.38} \def\yB{-1.42}

\node[font=\small\bfseries] at (\xL+\W/2, \yT+0.16) {firm size};

\draw[-{Stealth[length=3pt,width=2pt]}, line width=0.5pt, color=black!60]
  (\xL,\yB) -- (\xL,\yT+0.05);
\draw[-{Stealth[length=3pt,width=2pt]}, line width=0.5pt, color=black!60]
  (\xL,\yB) -- (\xR+0.12,\yB);
\node[rotate=90, font=\scriptsize, color=black!70, anchor=east]
  at (\xL-0.28,{\yT-0.23}) {$\ln S$};
\node[font=\scriptsize, color=black!70, below=3pt]
  at (\xL+\W/2,\yB) {$\ln s$};
\foreach \fr/\lb in {0.0/$s_0$, 0.333/$10s_0$, 0.667/$100s_0$, 1.0/$10^3s_0$}{
  \pgfmathsetmacro{\tx}{\xL+\fr*\W}
  \node[font=\tiny, color=black!55, below=1.5pt] at (\tx,\yB) {\lb};
}

% Zipf: straight line — black
\draw[color=black, line width=1.2pt, line cap=round]
  (\xL+0.04,\yT-0.10) -- (\xR-0.04,\yB+0.10);

\node[font=\tiny, color=black, anchor=center]
  at (10.798,\yT-0.35) {$\max S\,|\,\langle\ln s\rangle$};
\node[font=\tiny, color=black]
  at (\xL+\W*0.62,\yT-0.52) {slope $=-1$ (Zipf)};


%% ┄┄ PLOT 2: income ┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄

\pgfmathsetmacro{\yT}{0.38-\pitch}
\pgfmathsetmacro{\yB}{\yT-\H}

\node[font=\small\bfseries] at (\xL+\W/2,\yT+0.16) {household income};

\draw[-{Stealth[length=3pt,width=2pt]}, line width=0.5pt, color=black!60]
  (\xL,\yB) -- (\xL,\yT+0.05);
\draw[-{Stealth[length=3pt,width=2pt]}, line width=0.5pt, color=black!60]
  (\xL,\yB) -- (\xR+0.12,\yB);
\node[rotate=90, font=\scriptsize, color=black!70, anchor=east]
  at (\xL-0.28,{\yT-0.23}) {$\ln S$};
\node[font=\scriptsize, color=black!70, below=3pt]
  at (\xL+\W/2,\yB) {$\ln y$};
\foreach \fr/\lb in {0.0/$y_0$, 0.333/$10y_0$, 0.667/$100y_0$, 1.0/$10^3y_0$}{
  \pgfmathsetmacro{\tx}{\xL+\fr*\W}
  \node[font=\tiny, color=black!55, below=1.5pt] at (\tx,\yB) {\lb};
}

% x* dashed vertical
\draw[dashed, line width=0.4pt, color=black!40]
  (\xst,\yT+0.02) -- (\xst,\yB);

% BG income curve — black
\draw[color=black, line width=1.2pt, line cap=round, line join=round]
  (\xL+0.000*\W/2, \yT-0.112*\H)
  -- (\xL+0.143*\W/2, \yT-0.138*\H)
  -- (\xL+0.286*\W/2, \yT-0.172*\H)
  -- (\xL+0.429*\W/2, \yT-0.213*\H)
  -- (\xL+0.571*\W/2, \yT-0.263*\H)
  -- (\xL+0.714*\W/2, \yT-0.326*\H)
  -- (\xL+0.857*\W/2, \yT-0.404*\H)
  -- (\xst,           \yT-0.501*\H);

% Pareto income — black, uniform x-spacing, alpha_y=1.5
\draw[color=black, line width=1.2pt, line cap=round]
  (\xst,            \yT-0.5008*\H)
  -- (\xL+0.667*\W, \yT-0.6508*\H)
  -- (\xL+0.833*\W, \yT-0.8008*\H)
  -- (\xR-0.04,     \yT-0.9508*\H);

% T_y bracket
\pgfmathsetmacro{\tyw}{\f*\W*0.50}
\draw[{Stealth[length=2pt,width=1.5pt]}-{Stealth[length=2pt,width=1.5pt]},
      color=black, line width=0.5pt]
  (\xL+0.04,\yB+0.16) -- (\xL+0.04+\tyw,\yB+0.16);
\node[font=\tiny, color=black, above=0pt]
  at (\xL+0.04+\tyw/2,\yB+0.16) {$T_y$};

% Labels
\node[font=\tiny, color=black, anchor=west]
  at (\xL+0.36,\yT-0.21) {$\max S\,|\,\langle y\rangle$ \ BG};
\node[font=\tiny, color=black, anchor=west]
  at (\xst+0.10,\yT-0.21) {$\max S\,|\,\langle\ln y\rangle$ \ Pareto};
\node[font=\tiny, color=black, anchor=west]
  at (\xst+0.08, \yT-0.501*\H+0.12) {$-\alpha_y$};


%% ┄┄ PLOT 3: wealth ┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄┄

\pgfmathsetmacro{\yT}{0.38-2*\pitch}
\pgfmathsetmacro{\yB}{\yT-\H}

\node[font=\small\bfseries] at (\xL+\W/2,\yT+0.16) {household wealth};

\draw[-{Stealth[length=3pt,width=2pt]}, line width=0.5pt, color=black!60]
  (\xL,\yB) -- (\xL,\yT+0.05);
\draw[-{Stealth[length=3pt,width=2pt]}, line width=0.5pt, color=black!60]
  (\xL,\yB) -- (\xR+0.12,\yB);
\node[rotate=90, font=\scriptsize, color=black!70, anchor=east]
  at (\xL-0.28,{\yT-0.23}) {$\ln S$};
\node[font=\scriptsize, color=black!70, below=3pt]
  at (\xL+\W/2,\yB) {$\ln w$};
\foreach \fr/\lb in {0.0/$w_0$, 0.333/$10w_0$, 0.667/$100w_0$, 1.0/$10^3w_0$}{
  \pgfmathsetmacro{\tx}{\xL+\fr*\W}
  \node[font=\tiny, color=black!55, below=1.5pt] at (\tx,\yB) {\lb};
}

\draw[dashed, line width=0.4pt, color=black!40]
  (\xst,\yT+0.02) -- (\xst,\yB);

% BG wealth — black
\draw[color=black, line width=1.2pt, line cap=round, line join=round]
  (\xL+0.000*\W/2, \yT-0.167*\H)
  -- (\xL+0.143*\W/2, \yT-0.206*\H)
  -- (\xL+0.286*\W/2, \yT-0.256*\H)
  -- (\xL+0.429*\W/2, \yT-0.317*\H)
  -- (\xL+0.571*\W/2, \yT-0.393*\H)
  -- (\xL+0.714*\W/2, \yT-0.486*\H)
  -- (\xL+0.857*\W/2, \yT-0.603*\H)
  -- (\xst,           \yT-0.747*\H);

% Pareto wealth — black, uniform x-spacing, alpha_w=0.7
\draw[color=black, line width=1.2pt, line cap=round]
  (\xst,            \yT-0.7470*\H)
  -- (\xL+0.667*\W, \yT-0.8170*\H)
  -- (\xL+0.833*\W, \yT-0.8870*\H)
  -- (\xR-0.04,     \yT-0.9570*\H);

% T_w bracket (shorter than T_y)
\pgfmathsetmacro{\tww}{\f*\W*0.35}
\draw[{Stealth[length=2pt,width=1.5pt]}-{Stealth[length=2pt,width=1.5pt]},
      color=black, line width=0.5pt]
  (\xL+0.04,\yB+0.16) -- (\xL+0.04+\tww,\yB+0.16);
\node[font=\tiny, color=black, above=0pt]
  at (\xL+0.04+\tww/2,\yB+0.16) {$T_w$};

% Labels
\node[font=\tiny, color=black, anchor=west]
  at (\xL+0.36,\yT-0.21) {$\max S\,|\,\langle w\rangle$ \ BG};
\node[font=\tiny, color=black, anchor=west]
  at (\xst+0.10,\yT-0.21) {$\max S\,|\,\langle\ln w\rangle$ \ Pareto};
\node[font=\tiny, color=black, anchor=west]
  at (\xst+0.08, \yT-0.747*\H+0.12) {$-\alpha_w$};

% Boxed inequalities — both in wealth plot, black
\node[font=\scriptsize, color=black,
      draw=black, fill=white, rounded corners=2pt,
      inner sep=2pt, line width=0.4pt, anchor=north west]
  at (\xL+0.22, \yT-0.40*\H) {$T_w < T_y$};
\node[font=\scriptsize, color=black,
      draw=black, fill=white, rounded corners=2pt,
      inner sep=2pt, line width=0.4pt, anchor=north east]
  at (\xR-0.04, \yT-0.40*\H) {$\alpha_w < \alpha_y$};

%% ── Panel label ───────────────────────────────────────────
\node[font=\small] at (\xL+\W/2,-7.55) {(b)};

\end{tikzpicture}


==> Fig1_02.tex <==
\begin{tikzpicture}[x=1cm, y=1cm]

% ════════════════════════════════════════════════════════════
%  LEFT PANEL (a)
% ════════════════════════════════════════════════════════════

% (bounding box removed)

%% ── Sector boxes ──────────────────────────────────────────

% Firms
\draw[draw=bordergray, fill=boxgray, rounded corners=4pt, line width=0.4pt]
  (0.30, -0.42) rectangle (5.70, 0.42);
\node[font=\small, align=center] at (3.00, 0.14)
  {\textbf{Firms}};
\node[font=\scriptsize] at (3.00, -0.17)
  {Zipf size distribution};

% Households (outer) — white fill
\draw[draw=bordergray, fill=white, rounded corners=5pt, line width=0.4pt]
  (0.30, -4.485) rectangle (5.70, -1.985);
\node[font=\small] at (3.00, -2.255)
  {\textbf{Households}};

% Employees sub-box
\draw[draw=bordergray, fill=boxgray, rounded corners=3pt, line width=0.4pt]
  (0.45, -4.285) rectangle (2.75, -2.685);
\node[font=\footnotesize] at (1.60, -2.935)
  {\textbf{Employees}};
\node[font=\tiny] at (1.60, -3.285)
  {$\oplus$ additive wages};
\node[font=\tiny] at (1.60, -3.585)
  {BG income};
\node[font=\tiny] at (1.60, -3.905)
  {BG wealth};

% Owners sub-box
\draw[draw=bordergray, fill=boxgray, rounded corners=3pt, line width=0.4pt]
  (3.25, -4.285) rectangle (5.55, -2.685);
\node[font=\footnotesize] at (4.40, -2.935)
  {\textbf{Owners}};
\node[font=\tiny] at (4.40, -3.285)
  {$\otimes$ multiplicative};
\node[font=\tiny] at (4.40, -3.585)
  {Pareto income};
\node[font=\tiny] at (4.40, -3.905)
  {Pareto wealth};

% Government
\draw[draw=bordergray, fill=boxgray, rounded corners=4pt, line width=0.4pt]
  (0.30, -6.90) rectangle (5.70, -6.05);
\node[font=\small] at (3.00, -6.34)
  {\textbf{Government}};
\node[font=\scriptsize] at (3.00, -6.67)
  {fiscal flows (invariant)};

%% ── SOLID arrows ──────────────────────────────────────────

% Wages
\draw[solidarr] (1.60, -0.42) -- (1.60, -2.685);
\node[elabel] at (1.60, -1.202) {wages};

% Consumption
\draw[solidarr] (3.00, -1.985) -- (3.00, -0.42);
\node[elabel] at (3.00, -1.202) {consumption};

% Returns
\draw[solidarr] (4.40, -0.42) -- (4.40, -2.685);
\node[elabel] at (4.40, -1.202) {returns};

%% ── DASHED arrows ─────────────────────────────────────────

% HH taxes
\draw[dasharr] (3.00, -4.485) -- (3.00, -6.05);
\node[elabel] at (3.00, -5.268) {hh taxes};

% Firm taxes: right margin
\draw[dasharr]
  (5.70,  0.00) -- (6.25,  0.00)
               -- (6.25, -6.48)
               -- (5.70, -6.48);
\node[elabel, rotate=90] at (6.25, -3.24) {firm taxes};

% Spending: left margin
\draw[dasharr]
  (0.30, -6.48) -- (-0.25, -6.48)
               -- (-0.25,  0.00)
               -- ( 0.30,  0.00);
\node[elabel, rotate=90] at (-0.25, -3.24) {spending};

%% ── Panel label ───────────────────────────────────────────
\node[font=\small] at (3.00, -7.55) {(a)};


% ════════════════════════════════════════════════════════════
%  RIGHT PANEL (b)  — simulation output (Fig1_02)
% ════════════════════════════════════════════════════════════

% Replace hand-drawn curves with actual simulation figure
\node[anchor=center] at (9.85, -3.50) {%
  \includegraphics[width=6.0cm, height=8.0cm, keepaspectratio=false]{fig1_rhs_v2.pdf}%
};

%% ── Panel label ───────────────────────────────────────────
\node[font=\small] at (9.85,-7.55) {(b)};

\end{tikzpicture}

